Evidence of absorption dominating over scattering in light attenuation by nanodiamonds

We show an experimental evidence of the domination of absorption over scattering in absorbance spectra of detonation nanodiamonds. We perform the absorbance measurements on the UV-Vis spectrophotometer equipped with integrating sphere and compare them with conventional absorbance spectra. Additionally, we measure the scattering light intensity at the cuvette side wall (scattering at 90 degrees angle). The obtained experimental data were interpreted using the simulations of photon random walk in turbid media and Kubelka-Munk approach. The scattering cross sections and indicatrices were obtained by Mie theory. We discover that despite being very close to $\lambda^{-4}$ power law (like Rayleigh scattering) the light extinction by the primary 4 nm diamond crystallites is due to absorption only and scattering can be neglected. That is the reason why previously absorption and scattering contributions were confused. The scattering is governed only by the agglomerates of 100 nm and larger in size remaining in the hydrosols and their fraction can be effectively controlled by centrifugation. Only Mie theory reproduces correctly the close to $\lambda^{-2}$ scattering by the agglomerates accounting for the weird interplay between their size, fractal dimension, and dielectric properties. Finally, using the obtained absorbance spectra we estimate the fraction of non diamond phase in nanodiamonds and their agglomerates.

==> tmp_text.tex <==


%One can estimate the fraction of non-diamond phase in the primary crystallites from the value of : several percents.

%For this moment it is impossible to specify precisely the mechanism of absorption in the primary crystallites, but this is out of scope of present paper. The conclusion is that the absorption in nanodiamond hydrosols originates from disordered C network with sp$^{3-x}$ hybridization and clarification of its nature and creation of appropriate theoretical model is a challenge for the future studies of nanodiamonds.

% We can only  The goal of present paper was to show, how the contributions of absorption and scattering to DND optical density can be separated.





%Importantly, the plots can be approximated with sufficient quality for all $D_A \geq 200$nm. For filling factor $C_A \ll 1$ and small imaginary part of dielectric permittivity the following combinations are constant: $\sigma\scau\ml/c_A^2$ and $\sigma\absu\ml/c_A^3$. 

%Despite Eq. \eqref{eq_ODwith} and Eq. \eqref{eq_AscafromOD} are approximate, they have sufficient accuracy for extracting absorption and scattering contributions to OD from the obtained OD spectra with IS and without it.
%It is seen from an agreement between the curves (experimental data) and points (OD values prediction by the theory) in Figs. \ref{fig_ODZP_1} and \ref{fig_ODZP_2}. For Z02 sample (with very strong scattering and moderate absorption) Eq. \eqref{eq_ODwith} and Eq. \eqref{eq_AscafromOD} work worse, which is seen in Fig. X of the supplementary.



% due to importance of the scattering indicatrix and complicated diffusive photon trajectory in the medium.

The equation
\begin{equation}
\label{eq_ODwith}
\ODW\ml = \frac{A\absu\ml \cdot L}{\ln10}. 
\end{equation}
is correct only in the case of strong forward scattering: when all light gone from the cuvette goes to the sphere and no light goes to the side walls and backwards. Below we will see that its accuracy for the actual samples was of the order of 50\%.


%================================================

\subsection{Simple estimations of scattering and  based on data with sphere}

Optical density without IS writes as usually:

\begin{equation}
\label{eq_ODWO}
\ODWO\ml=\frac{A\scau\ml \cdot L+A\absu\ml \cdot L}{\ln10},
\end{equation}
where $A\absu\ml$ and $A\scau\ml$ are the contributions to the extinction coefficient of the hydrosol from absorption and scattering, respectively, and $L$ it the optical path in the cuvette. \footnote{e.g. for hydrosol with a number of particles per volume $n$ having cross sections $\sigma\absu\ml$ and $\sigma\scau\ml$ one writes $A\absu\ml = \sigma\absu\ml \cdot n$ and $A\scau\ml = \sigma\scau\ml \cdot n$. \green{This is the simplest case when the hydrosol contains the particles of a single size (unimodal distribution). In section \ref{sec_simulation} we use the bimodal distribution (two characteristic sizes) essentially required for the description of DND optical properties. The formulas for $A\scau\ml$ and $A\absu\ml$ will be naturally modified for the bimodal distribution: they will have the two terms corresponding to each size.}}

Now let us show how one can judge about absorption and scattering contributions based on the OD measurements with IS and without it. First one can obtain the total light intensity $I\WO\ml+I\sca\ml$ gone from the cuvette and driven to the detector by the IS as

\begin{equation}
\label{eq_Iwith}
I\WO\ml+ CONST \times I\sca\ml = I\refl \cdot \exp(-A\absu\ml \cdot \tilde{L}),
\end{equation}
where $\tilde{L}$ estimates the effective path of the light in the cuvette. In general case it not equal to the optical path in the cuvette size $L$ due to multiple scattering and diffusive trajectory, but in case of low absorption and scattering (or for dominating forward scattering) one can assume that $\tilde{L} = L$. In this assumption, combining Eq. \eqref{eq_Iwith} and Eq. \eqref{eq_2} one can write

\begin{equation}
\label{eq_ODwith}
\ODW\ml = \frac{A\absu\ml \cdot L}{\ln10}. 
\end{equation}

\textbf{Eq. (4) in fact is a Buger-Lambert-Beer law, but applied not for the single light path going along the spectrometer optical axis, but to all trajectories of scattered photons falling onto the IS surface. This is the peculiar origin for the difference between $L$ and $\tilde{L}$.}

Finally from Eqs. \eqref{eq_ODWO} and \eqref{eq_ODwith} one can derive that

\begin{equation}
\label{eq_AscafromOD}
\ODWO\ml - \ODW\ml = \frac{A\scau\ml \cdot L}{\ln10}.
\end{equation}

Eqs. \eqref{eq_ODWO} and \eqref{eq_AscafromOD} are not exact, but they are very useful for rapid estimation of contribution to extinction associated with scattering from OD measurements without IS and with it. If $\ODWO\ml \approx \ODW\ml$ one can conclude that the scattering is small with respect to absorption.



%=========================================




Substituting Eq (3) and Eq. (5) to the equation above one obtains the following estimation:

\begin{equation}
\label{eq_analTsca}
T\sca\ml = \exp(-A\absu\ml \cdot L)\cdot \left(1-\exp(-A\scau\ml \cdot L) \right) \approx \exp({-A\absu\ml L}) \cdot A\scau\ml L),
\end{equation}
which is valid at least for relatively for small scattering. To be simpler interpreted, this equation can be rewritten as follows:
\begin{equation}
\exp({-A\absu\ml L}) \cdot A\scau\ml L) = \exp({-A\absu\ml L/2}) \cdot A\scau\ml L) \cdot \exp({-A\absu\ml L/2}).
\end{equation}

The first multiplier in the right-hand part of the equation above shows that light attenuates due to absorption along the distance $L/2$ from the entering point to the cuvette center. The second multiplier says that the light scatters in the cuvette center and intensity of scattered light is proportional to scattering cross section (and thus to scattering contribution to optical density). Finally the light goes along $L/2$ from the cuvette center (where the scattering takes place) to the cuvette side wall (the third multiplier).


%==================================================================================



 This coincides with the proposed in Ref. \cite{dideikin2017rehybridization} mechanism of aggregates deagglomeration by removing the sp$^2$-like phase (highly absorbing) in the areas where the diamond nanoparticles touch each other in the crystallites. The mechanism of absorption by primary crystallites can be accounted by Urbach tail in the density of states. 





Fig. \ref{fig_Calc} shows the $T_{sca}$ value calculated from optical density spectra  without and with IS (see Fig. \ref{fig_Plus}, \ref{fig_Minus} and Fig. \ref{fig_0}) using Eq. \eqref{eq_TscaFromSphere}.


\begin{figure}
\includegraphics[width=0.5\textwidth]{ZM_Size.png}
\caption{\label{fig_ZM_Size} Distribution by scattered light intensity for Z- nanodiamond supernatant (upper panel) and precipitate (lower panel).}
\end{figure}

\begin{figure}
\includegraphics[width=0.5\textwidth]{Z0_Size.png}
\caption{\label{fig_ZO_Size} Distribution by scattered light intensity for Z0 nanodiamond supernatant (upper panel) and precipitate (lower panel).}
\end{figure}

\begin{figure}
\includegraphics[width=0.5\textwidth]{fig4.pdf}
\caption{\label{fig_Calc} Scattering intensities $T_{\mathbf{sca}}$ spectra for all samples calculated from optical density spectra without and with IS on the basis of Eq. \eqref{eq_TscaFromSphere}.}
\end{figure}

%spectra of scattering, absorption and t of Z+1 sample together with the OD spectra of Z+1 and Z+2 spectra measured without and with IS.


%Fig. \ref{fig_Plus}, \ref{fig_Minus} and Fig. \ref{fig_0} show she measured optical densities of samples Z+, Z- and Z0, respectively, without and with IS.






%\subsection{90 degree scattering, simulation results and separating }



the results of photon random walk simulations. 







%\subsection{Comparison with simulation}


Whereas, the simulation of the photon random walks allows to connect the 90 degree scattering spectra, optical density spectra without and with IS and contribution of the absorption and scattering to the total optical density. As a result the absorption and scattering contributions to optical density can be separated with sufficient accuracy.



\begin{table}[h]
\caption{The adjustement parameters used in the calculations and the plot features they control. All parameters except $m_A$ are common for all samples. \label{table2}}

\begin{tabular}{|l|c|>{\centering\arraybackslash}m{10cm}|}
  \hline
  Parameter & Value & Controlled feature of OD spectra \\
  \hline
  
  $P_P$ & -2.5  & Slope of OD curves for supernatants (Z+1,Z-1,Z01) governed mainly by absorption\\
  \hline
  $A_P$ & 0.15 & Magnitude of OD curves for supernatants governed mainly by absorption\\
  \hline
  $D_A$ & 200 nm  & Slope and magnitude of all OD curves (scattering and absorption) for precipitates (Z+2,Z-2,Z02) and $T_{sca}$ for supernatants\\
  \hline
  $P_A$ & -1 & Moderate (because of Mie limit) effect on the slope and magnitude of OD curves for precipitates (Z+2,Z-2,Z02) \\
  \hline
    $A_A$ & 1.05  & Magnitude of absorption contribution to OD and on amplitude  $T_{sca}$ for precipitates due to absorption of scattered light(see Eq. \eqref{eq_analTsca}).\\
\hline  
    $c_A$ & 0.13  & Slope and magnitude of scattering and absorption spectra for precipitates \\
  \hline
   $m_A$ & - & Contribution of scattering to OD and $T_{sca}$ for all samples \\
  \hline
\end{tabular}
\end{table}




%This figure (and the corresponding figures for Z- and Z0 samples in the supplementary) It exhibits the desired decomposition of OD spectra to absorption and scattering contributions.

%Eq. \eqref{eq_ODWO} was used for OD (total extinction) calculation and the two terms in this equation correspond to the scattering and absorption contributions. Absorption should be compared with $\ODW \ml$ (according to Eq. \eqref{eq_ODwith}) and scattering should be compared with $\ODWO-\ODW$ (according to Eq. \eqref{eq_AscafromOD}). Fig. \ref{fig_ODZP_2} shows the calculated in the same way OD spectra of Z+2 sample. Fig. \ref{fig_TscaZP} shows the scattering efficiency in terms of $T_{sca}$ obtained by the photon random walk simulation and from experiments. The results for Z- and Z0 samples are given in supplementary material.

%\textbf{The following parameters were adjusted. The agglomerate size $D_A$, constants in dielectric permittivities ($A_P$, $A_A$, $P_P$, and $P_A$), filling factor for agglomerates $c_A$ were the same for all studied samples (see Table \ref{table1}). The agglomerates mass fraction in the hydrosol $m_A$ was tuned for each sample separately (see Table \ref{table1}). From the first glance one can conclude that this amount of adjustment parameters is too large and tricky. But in fact it is comparable with the number of features of plots to be explained. One can refer these features as the slopes and magnitudes of Z+1 and Z+2 OD spectra without sphere and slopes and magnitudes of $T_{sca}$ (also for Z+1 and Z+2 samples): overall 8 features. This is the reason why the straightforward NLS parameter fitting method can not be used and manual tuning is required. The bottleneck is in the cumbersomeness of photon random walk simulation.}



%In the first approximation, the parameters fitting the procedure started with achieving agreement between theory OD measurements with IS and without it. Eqs. \eqref{eq_Ascattering} and \eqref{eq_Aabsorption} were substituted to Eq. \eqref{eq_ODwith} for absorption, to Eq. \eqref{eq_AscafromOD} for scattering and to Eq. \eqref{eq_ODWO} for total extinction. \textbf{It should be noticed that Eq. \eqref{eq_ODwith} for absorption and Eq. \eqref{eq_AscafromOD} are approximate and therefore the matching is obligatory only for $\ODWO$ (given by Eq. \eqref{eq_ODWO}) and for $T_{sca}$ (obtained by photon random walks simulation).} At the second step the parameters were tuned more fine for obtaining the agreement in terms of $T\sca$ (plotted in Fig. \ref{fig_TscaZP}), because $T\sca$ is much more sensitive quantity to alternating the parameters. This is due to the fact that according to Eq. \eqref{eq_analTsca} $T_{sca}$ contains the exponent of scattering attenuation coefficient, while by their nature the OD is linear in attenuation coefficient. This is the reason, why for more precise interpreting the experiments, it is better to operate in terms $T_{sca}$ and if possible provide the 90 degree scattering experiments.

%From to Fig. \ref{fig_ODZP_1} and Fig. \ref{fig_ODZP_2} one can see that Eqs. \eqref{eq_AscafromOD} and \eqref{eq_ODwith} despite their approximate nature provide the good approximation for separating the scattering contribution to total extinction. Finally, it is important to underscore the difference between the absorption by primary crystallites and their aggregates. It is impossible to fit the OD and $T_{sca}$ spectra with $A_P=A_A$ and $P_P=P_A$.


%The following assumptions are made. We use the trimodal distribution of diamond nanoparticles in the hydrosol. In this model in hydrosol there are the two species of nanoparticles: primary nanodiamond crystallites of the size $D_P=4$ nm \cite{osswald2009phonon,vul2006direct,aleksenskii1997diamond,aleksenskii1999structure,shenderova2011nitrogen,ozerin2008x,koniakhin2018ultracentrifugation} with the number of particles per volume concentration $n_P$ and the aggregates of the size $D_A\approx 200$ nm with the number of particles per volume concentration $n_A$. Finally the parameter $m_A$ controls the mass fraction of the aggregates in the DND powder and thus defines $n_A$ and $n_P$.

%The \textsc{Wolfram Mathematica} package \cite{mathematica2009wolfram} was used for performing the simulations and further analysis.

%For the scattering and absorption cross sections calculation the Mie theory \cite{mie1908beitrage,hulst1957light,bohren1983absorption} was used. The performed code precisely reproduces the yield of the Matzler \textsc{Matlab} code \cite{matzler2002matlab}. \textbf{The input parameters for the Mie theory are the particle dielectric permittivity (given by Eqs. \eqref{eq_eps_primary} and \eqref{eq_eps_aggr1}), nanoparticle diameter ($D_P$ and $D_A$), light wavelength in vacuum $\lambda$ and water dielectric permittivity. The yield of the Mie theory is the the absorption cross section $\sigma^{(abs)}$, scattering cross section $\sigma^{(sca)}$ and scattering indicatrix (the latter is given in the supplementary materials in Fig. S4).} For the 4 nm primary crystallites the absorption and scattering cross sections are denoted as $\sigma_P\absu\ml$ and $\sigma_P\scau\ml$, respectively. For the large aggregates the scattering and absorption cross sections are $\sigma_A\scau\mu$ and $\sigma_A\absu\ml$, respectively. Contribution of primary particles to scattering in the hydrosol is negligible for all reasonable values of adjustment parameters: $n_P \cdot \sigma_P\scau\ml \ll n_A \cdot \sigma_A\scau\ml$.

%\textbf{The number of primary crystallites and aggregates per volume ($n_P$ and $n_A$, respectively) are calculated via the total diamond weight fraction WT2 listed in third column of Table \ref{table1} and the adjustment parameters: diameters $D_P$ and $D_A$, agglomerates mass fraction $m_A$ and filling factor $c_A$.}


%Also the photon is absorbed and excluded when it reaches the cuvette wall off the ''detector regions'', placed in the centers of the right wall and other 4 side walls. Obviously the detectors at the 4 side walls correspond to $T_{sca}$ value, while the detector at the right wall corresponds to measuring the conventional optical density $A_{WO}$.


%and changes its propagation direction according to the scattering indicatrix calculated with Mie theory (the example of such indicatrix is given in the supplementary materials). 

%In the end of the simulation the photon is absorbed, reaches side wall detectors or reaches the right side detector. The effective 90 degree transmission defined above is calculated as $T_{90} = N_{side}/N_{tot}$, where $N_{side}$ is the number of photons reached the side ''detector regions'' and $N_{tot}$ is the total amount of photons (simulation runs). For each wavelength $10^5$ runs were made.



%In the same manner $A_{WO} = -\log_{10} N_{right}/N_{tot}$, where $N_{right}$ is the number of photons reached the right ''detector region''. This value was compared with the experimental one. 




%These figures contain the data of all 6 samples (overall 12 curves in each), is necessary to provide the possibility to compare between the samples. In the next section and in the Supplementary Materials the information will be given for each sample separately and compared with the predictions of the theory.

%\textbf{Curves from this plot are depicted separately in figures below for Z+, Z- and Z0 samples (supernatants and precipitates).}}

%Let us analyze now solely the experimental results depicted in \ref{fig_ODZP_1}, Fig. \ref{fig_ODZP_2}, and Fig. \ref{fig_TscaZP}.

%One sees that for supernatants of disagglomerated diamond types (samples Z+1, Z-1) OD spectra without and with IS nearly coincides. According to Eq. \eqref{eq_AscafromOD} it means that the scattered light intensity is small and main contribution is from absorption. On the contrary for all precipitates (samples Z+2,Z-2,Z02) the difference with and without sphere is significant. The difference is also tangible for Z01 sample, because it lacks the disagglomeration procedure and intensively scattering agglomerates remain in the hydrosol.

%because of a lot of light is gone out of the cuvette and collected by the IS.
